PrideMM: A Solver for Relaxed Memory Models

Relaxed memory models are notoriously delicate. To ease their study, several ad hoc simulators have been developed for axiomatic memory models. We show how axiomatic memory models can be simulated using a solver for $\exists$SO. Further, we show how memory models based on event structures can be simulated using a solver for MSO. Finally, we present a solver for SO, built on top of QBF solvers.

==> results_table.tex <==
% File:  results_table.tex
% Author: mikolas
% Created on: Tue, Jan 23, 2018 15:29:38
% Copyright (C) 2018, Mikolas Janota
\begin{table}[th]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        instance         & QFM & QFUN & QuAbS & CAQE (CNF) \\
        \hline
        jctc1 &&&&\\\hline
        jctc2 &&&&\\\hline
        jctc3 &&&&\\\hline
        jctc4 &&&&\\\hline
        jctc5 &&&&\\\hline
        jctc5 &&&&\\\hline
        jctc6 &&&&\\\hline
        jctc7 &&&&\\\hline
        jctc8 &&&&\\\hline
        jctc9 &&&&\\\hline
        jctc10 &&&&\\\hline
        jctc11 &&&&\\\hline
        jctc12 &&&&\\\hline
        jctc13 &&&&\\\hline
        jctc14 &&&&\\\hline
        jctc15 &&&&\\\hline
        jctc15 &&&&\\\hline
        jctc16 &&&&\\\hline
        jctc17 &&&&\\\hline
        jctc18 &&&&\\\hline
    \end{tabular}
    \vspace{1em}
    \caption{Table}\label{tab:res}
\end{table}

